CasModaTest: A Cascaded and Model-agnostic Self-directed Framework for Unit Test Generation

Though many machine learning (ML)-based unit testing generation approaches have been proposed and indeed achieved remarkable performance, they still have several limitations in effectiveness and practical usage. More precisely, existing ML-based approaches (1) generate partial content of a unit test, mainly focusing on test oracle generation; (2) mismatch the test prefix with the test oracle semantically; and (3) are highly bound with the close-sourced model, eventually damaging data security. We propose CasModaTest, a cascaded, model-agnostic, and end-to-end unit test generation framework, to alleviate the above limitations with two cascaded stages: test prefix generation and test oracle generation. Then, we manually build large-scale demo pools to provide CasModaTest with high-quality test prefixes and test oracles examples. Finally, CasModaTest automatically assembles the generated test prefixes and test oracles and compiles or executes them to check their effectiveness, optionally appending with several attempts to fix the errors occurring in compiling and executing phases. To evaluate the effectiveness of CasModaTest, we conduct large-scale experiments on a widely used dataset (Defects4J) and compare it with four state-of-the-art (SOTA) approaches by considering two performance measures. The experimental results indicate that CasModaTest outperforms all SOTAs with a substantial improvement (i.e., 60.62%-352.55% in terms of accuracy, 2.83%-87.27% in terms of focal method coverage). Besides, we also conduct experiments of CasModaTest on different open-source LLMs and find that CasModaTest can also achieve significant improvements over SOTAs (39.82%-293.96% and 9.25%-98.95% in terms of accuracy and focal method coverage, respectively) in end-to-end unit test generation

==> sections/RQ4.tex <==
% Note: Removed RQ4 for now

\subsection{RQ4: Impacts of Instruction in Prompt}
\label{lab:rq4}

%How does the performance vary based on the level of specificity of the instructions?



\phead{Motivation.}
%\xyw{Many case studies have focused on exploring the effectiveness of prompts in harnessing the capabilities of large language models from a natural language perspective. It has been found that the level of precision in conveying intent significantly influences the performance of models.}
Prior studies find that the proper design of prompts can significantly improve the performance of LLMs in the tasks of code intelligence~\cite{cuiyungao_prompt_fse2022,cuiyungao_prompt_tse2023}.
In this RQ, we study the impact of two different designs of prompts, with different levels of specificity, on the performance of unit test generation. 




\phead{Approach.}
%We examine the impact of two sets of instructions with varying levels of specificity on performance from the perspective of instruction tuning.

\xyw{
In few-shot learning, a prompt is the final form of input into a large model. The prompt we designed consists of natural language instruction, code demonstrations, and the final tested content. 
}

\xyw{
Natural language instructions are placed at the very beginning of the prompt to describe the tasks that the model is expected to complete. They could be understood by models trained on English. We have designed two sets of instructions with different levels of specificity for \toolname$_{GPT3.5}$. In the preliminary version, the instruction in the prefix generation stage are to “Generate test input using the following Java code,” and in the oracle generation stage, to “Generate oracle using the following Java code.” In the precise version, the instruction in the prefix generation stage are to "Your task now is only to construct the test inputs, not the test assertions. Use \texttt{CLASS\_CONSTRUCTOR} to get \texttt{CLASS\_NAME}, then call \texttt{TEST\_METHOD\_NAME}. Use java without comments.", and in the oracle generation stage, to "Your task now is to generate a test assertion to replace the \texttt{<{OraclePlaceHolder}>} in \texttt{UNIT\_TEST}. Only variables that occur after the last \texttt{UNIT\_TEST} can be used. Use java without comments.". 
}


%在prefix和oracle生成阶段，提示词中都有一段自然语言指令，位于5个样例的前方，设计了简单的(vanilla)和详细的(well-crafted)两组指令
% prefix generation stage 
% instruction_dict = {
%     "vanilla": "Generate test input in the following java code:\n",
%     "well_crafted": "Your task now is only to construct the test inputs, not the test assertions. Use CLASS_CONSTRUCTOR to get CLASS_NAME, then call TEST_METHOD_NAME. Use java without comments. End your reply with END_OF_DEMO.\n"
% }
% oracle generationstage 
% instruction_dict = {
%     "vanilla": "Generate oracle in the following java code:\n",
%     "well_crafted": "Your task now is to generate a test assertion to replace the <OraclePlaceHolder> in UNIT_TEST. Only variables that occur after the last UNIT_TEST can be used. Use java without comments. End your reply with END_OF_DEMO.\n"
% }
% vanilla版本的指令是非常模糊的，只要求跟随例子生成测试输入/预言
% well-crafted版本的指令在prefix生成阶段，指定了应该使用类构造器签名来实例化类，再用实例化出的类来调用方法。在oracle生成阶段说明了生成一句测试断言(实际中LLM一般不会只生成一句)来取代预言占位符，并且只能使用前面的过程已经定义过的变量。最后，两个阶段都说明了不要注释，并且以定义好的分隔符结尾，这样LLM知道何时应该停下。
% 其余都一样


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[!htbp]
  \centering
  \caption{Comparison between different instructions}
  \resizebox{\linewidth}{!}
  {
    \begin{tabular}{lr|rr|rr}
    \toprule
        \multirow{2}[1]{*}{\textbf{Projects}}     & \multirow{2}[1]{*}{\textbf{\# Query}}     & \multicolumn{2}{c|}{\textbf{\% Accuracy}} & \multicolumn{2}{c}{\textbf{\% Focal Method Coverage}} \\
    \cmidrule{3-6}
    & & {\textbf{Well-Crafted}} & {\textbf{Vanilla}} & {\textbf{Well-Crafted}} & {\textbf{Vanilla}} \\
    \midrule
    Cli   & 645   & \textbf{58.29\%} & 54.88\% & \textbf{61.98\%} & 58.76\% \\
   
    Csv   & 373   & \textbf{69.17\%} & 64.88\% & \textbf{77.42\%} & 74.53\% \\

    Gson  & 220   & 63.18\% & \textbf{65.00\%} & 63.35\% & \textbf{68.18\%} \\

    Chart & 1328  & \textbf{76.66\%} & 75.60\% & \textbf{82.55\%} & 80.80\% \\
    Lang  & 2712  & \textbf{84.13\%} & 81.78\% & \textbf{88.49\%} & 85.40\% \\
    \midrule
    \rowcolor{lightgray} All   & 5278  & \textbf{77.16\%} & 75.04\% & \textbf{81.93\%} & 79.50\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:rq4_diff_instructions}%
\end{table}%






\phead{Results.}
Table~\ref{tab:rq4_diff_instructions} shows the comparative performance of unit test case generation using Well-Crafted and Vanilla prompts, evaluated based on accuracy and focal method coverage across five distinct projects.

\textbf{Accuracy.} The Well-Crafted prompts achieve better performance than the Vanilla prompts in accuracy across the majority of the projects.
For example, in Cli project, the Well-Crafted prompt design achieves an accuracy of 58.29\%, surpassing the Vanilla design by 3.41\%. 
Similarly, in the Csv project, the Well-Crafted design leads with an accuracy of 69.17\%, outperforming the Vanilla design by 4.29\%. 
However, the Gson project presents an intriguing deviation where the Vanilla design achieves a slightly higher accuracy of 65.00\%, compared to the Well-Crafted design's 63.18\%. 
On aggregating the results across all projects, the Well-Crafted design leads with an overall accuracy of 77.16\%, which is 2.12\% higher than the Vanilla design.

\textbf{Focal Method Coverage.} In terms of focal method coverage, the majority of projects exhibit superior performance with Well-Crafted prompts compared with Vanilla ones.
In the Cli project, the Well-Crafted design achieves a coverage of 61.98\%, outperforming the Vanilla design by 3.22\%. 
This trend continues in the Csv and Chart projects, where the Well-Crafted design surpasses the Vanilla design by 2.89\% and 1.75\%, respectively. 
However, the Gson project showcases the strength of the Vanilla design with a coverage of 68.18\%, which is 4.83\% higher than the Well-Crafted design. 
When considering the results across all projects, the Well-Crafted design achieves an overall coverage of 81.93\%, which is 2.43\% higher than the Vanilla design.


\intuition{{\bf Summary of RQ4}: The experimental results underscore the superior performance of Well-Crafted prompts in unit test case generation across both accuracy and focal method coverage metrics. While the Gson project serves as an exception, the overall trend across the majority of projects clearly highlights the enhanced efficacy of well-crafted prompts over the vanilla ones.}
